TypeFly: Flying Drones with Large Language Model

Recent advancements in robot control using large language models (LLMs) have demonstrated significant potential, primarily due to LLMs' capabilities to understand natural language commands and generate executable plans in various languages. However, in real-time and interactive applications involving mobile robots, particularly drones, the sequential token generation process inherent to LLMs introduces substantial latency, i.e. response time, in control plan generation. In this paper, we present a system called ChatFly that tackles this problem using a combination of a novel programming language called MiniSpec and its runtime to reduce the plan generation time and drone response time. That is, instead of asking an LLM to write a program (robotic plan) in the popular but verbose Python, ChatFly gets it to do it in MiniSpec specially designed for token efficiency and stream interpretation. Using a set of challenging drone tasks, we show that design choices made by ChatFly can reduce up to 62% response time and provide a more consistent user experience, enabling responsive and intelligent LLM-based drone control with efficient completion.

==> sections/design-llmc.tex <==
% 
\section{Prompt Generation 
%with Scene-based Incremental Planning and Low-level Skill Triggered Replanning
}\label{sec:LLMController}
% \nl{how about merge section5 here and reorganize as follows: 4.4.1 Prompt for control, 4.4.2 Prompt for probe}
% \lin{I like this idea.}

% \nl{how about move the description of prompt to the next section}
% \lin{Agreed}
% \sout{We note that the new Planning prompt has the same task description; because it also includes the original plan and its execution status, the \llm will understand that how much of the plan has been executed and produce a new plan accordingly.}

\lin{Maybe a better section title than LLMController?}
\nl{ How about Drone Plan Generation}
%and make this section one subsection of Section 5, and the focus of this subsection could be how to generate the MiniSpec Plan with LLM(include plan and replan, leave prompt for probe to the introduction of probe?)

\system utilizes in-context learning to generate \lang \plan with LLM for drone control.
To ensure accurate, concise, and efficient \lang \plan generation, we integrate a \llmc module into the \system. The primary function of the \llmc module is to prepare and transmit prompts to the Remote LLM. We will also discuss our prompt design for plan generation in this section.

% \subsection{\llmc}
% \nl{Since we remove most part of this section, the following text is no longer applicable. How about deleting it?}
% \sout{We have three objectives in designing \llmc: (1) efficient use of the \llm, which can be slow for output generation; (2) improving the success rate of the plan when the task involves environment that is unseen during the initial planning; and (3) efficient task completion by the drone, which is constrained by flight time and usability. Toward achieving these three objectives, \llmc not only must prompt the \llm carefully (See \S\ref{sec:semantics}) but also effectively use the two special skills, \code{probe} and \code{replan}, to engage the \llm in plan execution.}

% \lina{This needs to be updated due to the change in execution modes}
% The \llmc can be represented by a three-state machine and stay in Wait when there is no task. Whenever the \llmc receives a \taskd from the user or a \code{replan} command from \langI, it enters the Planning state. It generates a rather long prompt to be described in \S\ref{sec:semantics}. 
% Once the prompt is generated, it enters the Execution state for sending the prompt to the Remote LLM. 
%On receiving the \plan, our \langI will conduct a syntax verification. Should this check be unsuccessful, the \llmc incorporates the syntax report into the prompt and retries Planning. 
% If the \langI invokes \code{replan}, the \llmc will instruct the \llm to plan again. 
% The cycle continues until the number of retries surpasses the predetermined threshold.

%that consists of the provided task description, the scene description from the \ve, system skill description, and the history of plan (if applicable), along with the prompt engineering


% \lin{Note that LLMC does not receive plans from the LLM as we revise Figure 1. Plans go to interpreter directly. LLMC only prepares and sends prompts}
% \nl{Move some sentences to the previous paragraph, shall we remove this paragraph?}
% Once the \llmc receives a valid \lang \plan from the \llm, it enters the Execution state. Because the \plan is a program in \lang, the \llmc employs an \langI to translate it into Python code and execute it. % In the event of a failed interpretation, the \llmc gathers the error report, incorporates it into a new Planning prompt and tries planning again. 
% If the \plan invokes \code{replan}, the \llmc will instruct the \llm to plan again. 
% The \llmc also monitors the plan execution and may inject \code{replan}.
% If the \plan invokes \code{probe(question: str)}, the \llmc consults the \llm with an execution prompt, which includes the ``question'', the latest \scened, and some guides to help \llm generate concise responses with a specific format. By \lang's design, a \plan always terminates.

% \begin{figure}[t]
% \begin{lstlisting}[language=Python]
% 8{_1=p('Any edible target here?');_1!=True{g(_1);->True}tc(45)}->False
% \end{lstlisting}

% \begin{lstlisting}[language=Python, label={code-plan-example}, caption={\textmd{\small Example \code{plan}s produced by the LLM (GPT-4) with (top) and without (bottom) \spskill skill for the task "Find something edible". \code{s} and \code{q} are the abbrevations for \code{sweeping} and \spskill, respectively.}}, escapechar=|]
% ?s('apple')==True{g('apple')->True}
% ?s('cake')==True{g('cake')->True}
% ?s('sandwich')==True{g('sandwich')->True}
% ?s('orange')==True{g('orange')->True}
% ->False
% \end{lstlisting}
% \vspace{-2em}
% \end{figure}

%We next explain how \code{replan} and \code{probe} work.


\input{sections/design-semantics}


==> sections/design-semantics.tex <==
% \subsection{Prompt Engineering}
% \label{sec:semantics}
%We next describe the techniques used by the Planning prompts.
% \subsection{Prompt Design}
\label{sec:semantics}
% \system leverages the \llm's few-shot learning capability to generate \lang \plan.

%prompt include guidance, minispec syntax, minispec skill sets, examples, scene description, task description, the history of the plan

\llmc constructs a comprehensive prompt that incorporates several essential elements. For drone control tasks, the prompt integrates the user's task description with current scene information from \ve. To generate the plan using \lang, we include a detailed description of the language's skill set and syntax. Additionally, a list of examples is provided to demonstrate how \lang can be used to formulate executable solutions that meet the task objectives. In scenarios requiring replanning, the prompt also includes the history of the previous plan, enabling the LLM to determine the extent of plan execution and generate a subsequent plan accordingly.


% To avoid expanding the output token number, which dominates the inference latency in our application, while maintaining the semantic correctness of the \plan, we provide rich context, a list of planning examples with detailed reasoning, and several optimizations in the prompt to overcome the limitations of \llm's reasoning ability without CoT or Think-Step-by-Step.

% we include the following optimizations in Planning prompts. They play an important role in improving task success as reported in \S\ref{sec:eval_p-prompt}.


\nl{add citation for step-by-step}
"Chain-of-Thought" \cite{wang2023arxiv} and "Think-Step-by-Step" are widely used in prompt design to enhance the accuracy of LLM generation. However, these approaches will also lead to huge plan generation time since they need to generate a long reasoning procedure before the plan generation. To maintain the semantic correctness of the plan while avoiding substantial delays in generation for reasoning, we have devised optimization guidance within our prompts. This approach eliminates the need for the LLM to generate an extensive reasoning procedure. Our guidance aids the LLM in more effectively processing scene and task descriptions and enhances its comprehension of the usage of language skills, thus offering a more efficient alternative to traditional methods. In the following, we will detail the design of our optimized guidance in the prompt.

%We note that the new Planning prompt has the same task description; because it also includes the original plan and its execution status, the \llm will understand that how much of the plan has been executed and produce a new plan accordingly.



% While the user is ultimately responsible for the semantic correctness of a \plan, \system features several optimizations that aim at overcoming the limitations of both the human user and the \llm.


\textit{Guide for Task Descriptions Reasoning}:~~
A precise \taskd is critical for the \llm to produce a correct \plan. 
Our experience shows that \taskds provided by a human user can be vague and ambiguous, leading the \llm to produce incorrect \plans. Leveraging \LLM's language capability, \system, specifically the \llmc, incorporates Guide 1 in the \autoref{prompt-rules} to ask the \llm not to produce a \plan if it considers the \taskd as described in vague or grammatically incorrect English. Instead, the \llm will refine the \taskd and ask the user to confirm using the \code{log} skill. Here is an example:

\vspace{0.5em}
\begin{customframe}
\textbf{User Input:} \textit{Find a btle in the kitchen.}\\
\textbf{\system:} \textit{Did you mean "bottle"? Please confirm the object.}
% \hspace*{4em}
\end{customframe}

\begin{figure}[t]
% \begin{lstlisting}[label={prompt-rules}, caption={\textmd{Task reasoning guides embedded in the planning prompt.}}, escapechar=|]
\begin{lstlisting}[label={prompt-rules}, caption={\textmd{\small Reasoning guides embedded in the Planning prompt}}, escapeinside={(*@}{@*)}]
(*@\color{typeflyred} Handling Typos and Ambiguous Language@*): When encountering typos or vague language in user inputs, strive to clarify and correct these ambiguities. If a typo is evident, adjust the input to reflect the most likely intended meaning. For vague or unclear expressions, seek additional information or use context clues from the scene and task descriptions to infer the most probable interpretation. 
(*@\color{typeflyred} Analytical Scene and Task Assessment@*): Evaluate the scene and task critically. If a specific condition or requirement is clearly deduced from the scene description, generate the corresponding action directly.
(*@\color{typeflyred}Relevance to Current Scene@*): When considering user tasks, assess their relevance to the current scene. If a task does not pertain to the existing scene, disregard any details from the current scene in formulating your response.
(*@\color{typeflyred} Extraction of Key Information@*): Extract 'object_name' arguments or answers to questions primarily from the 'scene description'. If the necessary information is not present in the current scene, use the probe 'p(question)', to determine the 'object_name' or answer subsequently.
(*@\color{typeflyred} Handling Replan@*): When previous response and execution status are provided, it means part of the task has been executed. In this case, the system should replan the remaining task based on the current scene and the previous response.
\end{lstlisting}
%\vspace{-1em}
\end{figure}
 
\textit{Guides for Scene Reasoning and Use of \emph{\code{probe}} and \emph{\code{probe}}}:~~
We include another three task reasoning guides in Planning prompts, shown in \autoref{prompt-rules}, to help the LLM better understand the \taskd and generate good plans. Guides 2 and 3 are about scene reasoning. They emphasize the close relationship between task and scene descriptions. Guide 4 provides insight into proper use of \spskill: only when the required information is missing in the current scene, \spskill should be called with an appropriate question. Guide 5 teaches the system how to respond to a Planning prompt invoked by \code{replan}.

%\textit{Few-shot Examples}:~~
%LLMs are recognized for their few-shot learning capabilities, meaning they can effectively learn and adapt from a limited set of examples. 
%We provide a small but comprehensive collection of examples that demonstrate the broad range of system skills available with detailed reasoning for the \llm to learn from.

\begin{comment}
\subsection{Skill Design and Usage}
\label{sec:skilldesign}
During the design of system skills, we consider the following factors to ensure that the \llm can generate a correct and efficient \plan. 

\textit{Easy Argument Passing.} We design a skill so that it has as few arguments as possible and the values of arguments can be found in the prompt. This makes it easier for the \llm to correctly invoke the skill.
For example, the aptest skill for the \llm to use when queried with "Can you move forward by 1 meter?" would be \code{move\_forward(distance\_in\_} \code{meter: float)}. This function not only aligns seamlessly with the task but its singular argument can be directly discerned from the description's mention of "1". In contrast, less suitable system skills might include \code{move(x: float, y: float, z: float)} due to its inclusion of extraneous arguments, or \code{move\_forward(distance\_in\_mile: float)}, which introduces unnecessary unit conversion.

\textit{Provide Options, not Range.} We leverage the LLM's strength of pattern recognition while eschewing its weakness in arithmetic.
When dealing with a potentially numerical argument, we approximate by turning its range into options. For example, when prompted with \task{Go to the door quickly}, \code{set\_speed(s-}\code{peed: str)} with predefined options of \code{[slow, medium, fast]} is more likely to work as expected than \code{set\_speed(value: int)} with a range of $[0\sim 100]$.
The authors of \cite{wang2023arxiv}, \cite{kojima2023arxiv}, and our own experience show that prompting LLMs without Chain-of-Thought (CoT) or Think-Step-by-Step on calculation related problems would result in erroneous responses. Yet including CoT would significantly increase the LLM response, which is opposite to our goal of latency efficiency.
When numerical arguments are inevitable, we design the skill so that their values are more likely to be present in the scene description. For example, when designing a skill to navigate the drone to approach an object, we would use \code{move\_to(location)} instead of \code{move\_by(displacement)} since the object's location can be found in the scene description but displacement requires extra calculation.

\gc{add the skill usage section}
\textit{Skill Usage} In the planning prompt, we encourage the \llm to use high-level skills as much as possible. This is because high-level skills are user verified and tested functions that will commonly be used in the \plans. For example, the \llmc will encourage the \llm to use \code{sweeping} to find an object instead of using \code{turn\_cw} and \code{is\_visible} in sequence.

\end{comment}

\textit{Trade-off Between Cost and Latency}:~~
To achieve the optimal latency and accuracy, \system uses a big prompt to guide the \llm to generate the least number of tokens while maintaining the semantic correctness of the \plan. Such a design is based on our observation (as shown in \autoref{fig:gpt4-latency}) that the inference latency differs greatly for input and output tokens. The drawback of this design is that, with the current cost model of LLMs, \system would result in a higher cost than a system that uses a smaller prompt. However, we observe that works like \cite{gim2023prompt} have shown the potential of reducing the cost for LLMs service of a big structured prompt by reusing the prompt cache. We believe that the cost of \system will be reduced in the future.

==> sections/recycle.tex <==
\textit{Task 1}: 
As illustrated as follows, %the top block is the simplified planning prompt and the bottom block is the \plan returned by \llm. 
the \plan simply turns the drone clockwise by 180 degrees, orients the drone to the person, and approaches it. 
% in \autoref{lst:task-1}, 

\begin{figure}[h]
{\footnotesize Task 1: Planning Prompt}
\begin{lstlisting}[escapeinside={(*@}{@*)}]
scene description:
(*@\color{typeflypurple}[...]@*)
task description:
(*@\color{typeflygreen}Go to the person behind you.@*)
\end{lstlisting}
% \begin{lstlisting}[caption={\textmd{\smaller Scene Desc., Task Desc., and Plan for task 1.}}, label={lst:task-1}]
{\footnotesize Plan}
\begin{lstlisting}[label={lst:task-1}]
tc,180;o,person;a
\end{lstlisting}
\end{figure}


\textit{Task 5}: As illustrated below, the plan starts with a loop of 8 times. In each iteration, it uses \spskill to check "yellow and sweet target," which is a banana in our case. If the target object is found, it will first orient the drone to and approach the target before returning \code{True}. Otherwise, the drone will turn clockwise for 45 degrees and start the next iteration. If the loop finishes, which means no target object is found, the \plan will return \code{False}.

\begin{figure}[h]
{\footnotesize Task 5: Planning Prompt}
\begin{lstlisting}[escapeinside={(*@}{@*)}]
scene description:
(*@\color{typeflypurple}[lemon\_2 x:0.2 y:0.71 width: 0.11 height:0.12, ...]@*)
task description:
(*@\color{typeflygreen}Find something yellow and sweet.@*)
\end{lstlisting}
{\footnotesize Plan}
\begin{lstlisting}[label={lst:task-5}]
8{_1=p('what's the yellow and sweet target?');?_1!=False{o,_1;a;->True}tc,45}->False
\end{lstlisting}
\end{figure}

\textit{Task 9}: As illustrated below, the plan first uses \spskill to check the number of people in sight. Then it does a comparison to decide whether to go to the most left person. Additionally, \prog{GPT4} successfully identifies which person is the leftmost. 
%We note that \system does not support memory for now, if it does, we can extend this task to \task{Scan the room and if you can see more than 2 people, go to the first person you seen}.
% in \autoref{lst:task-9}

\begin{figure}[h]
{\footnotesize Task 9: Planning Prompt}
\begin{lstlisting}[escapeinside={(*@}{@*)}]
scene description:
(*@\color{typeflypurple}[person\_2 x:0.22 y:0.5 width:0.43 height:0.7, person\_1 x:0.37 y:0.54 width:0.47 height:0.56, person\_3 x:0.76 y:0.65 width:0.35 height:0.71, ...]@*)
task description:
(*@\color{typeflygreen}If you can see more than two people, then turn to the leftmost person you see.@*)
\end{lstlisting}
{\footnotesize Plan}
\begin{lstlisting}[label={lst:task-9}]
_1=p('how many people are there?');?_1>2{o,person_2;a}
\end{lstlisting}
\end{figure}
